Optimal Decision Tree and Adaptive Submodular Ranking with Noisy Outcomes

In pool-based active learning, the learner is given an unlabeled data set and aims to efficiently learn the unknown hypothesis by querying the labels of the data points. This can be formulated as the classical Optimal Decision Tree (ODT) problem: Given a set of tests, a set of hypotheses, and an outcome for each pair of test and hypothesis, our objective is to find a low-cost testing procedure (i.e., decision tree) that identifies the true hypothesis. This optimization problem has been extensively studied under the assumption that each test generates a deterministic outcome. However, in numerous applications, for example, clinical trials, the outcomes may be uncertain, which renders the ideas from the deterministic setting invalid. In this work, we study a fundamental variant of the ODT problem in which some test outcomes are noisy, even in the more general case where the noise is persistent, i.e., repeating a test gives the same noisy output. Our approximation algorithms provide guarantees that are nearly best possible and hold for the general case of a large number of noisy outcomes per test or per hypothesis where the performance degrades continuously with this number. We numerically evaluated our algorithms for identifying toxic chemicals and learning linear classifiers, and observed that our algorithms have costs very close to the information-theoretic minimum.

==> cover_letter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}
\input{common_files/abbr_su}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Optimal Decision Tree with Noisy Outcomes}'' to the \emph{Journal of Machine Learning Research}.
% Our manuscript studies the problem of  \red{Optimal Decision Tree with Noisy Outcomes (ODTN)}, this problem is important because of \red{A, B, and C}.
This paper substantially extends its preliminary version, which appeared in {\em The Proceedings of the Thirty-third Conference on Neural Information Processing Systems} \red{(NeurIPS'19)}, in the following ways.
\benum 
\item {\bf Exposition.} We significantly improved the presentation of the paper.
\benum
\item {\bf Proof Sketches.} Proofs In the NeurIPS version were relegated to the appendix. 
In this version, we provide a proof sketch for every result directly in the main body.
We hope that this offers the reader a comprehensible grasp of the core ideas, without delving into the formal proof.
\item {\bf Revised Introduction.} We revised the Introduction to incorporate discussions resulting from the NeurIPS presentation and better articulate the positioning of our problem in the literature.
\item {\bf Complete proofs.} The NeurIPS version only included the proofs of a subset of results that are most crucial to understanding the results. In this version, we present formal proofs for all results.
\eenum
\item {\bf Beyond binary outcomes:} The NeurIPS version assumes that the outcome is binary. 
In this version, we extend our analysis to handle arbitrary finite outcome space. 
\item {\bf The ASRN problem:} We introduce a novel problem called {\em Adaptive Submodular Ranking with Noise} (ASRN) which generalizes both the ASR problem (Navidi et al., {\em Oper. Res.} 2020) and the classical Optimal Decision Tree (ODT) problem. We present the following results:
\benum 
\item {\bf Non-adaptive setting:} 
An $O(\log \frac m\eps)$-\apxn\ for the Non-adaptive version, where $m$ is the number of \submod\ \func s and $\eps$ is the separability of those \func s, and 
\item {\bf Adaptive setting:} 
An $O(\min\{c\log |\Omg|, r\} + \log \frac m\eps)$-\apxn\ for the adaptive version, where $r$ and $c$ measure the noise level and $\Omg$ is the outcome space.
\eenum
\eenum


We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item \red{Vehab Mirokni, Google (mirokni@google.com)}
    \item \red{Stefanie Jagelka, MIT (stefje@csail.mit.edu)}
    \item \red{Shipra Agarwal, Columbia University, (sa3305@columbia.edu)}
    \item \red{Kevin Jamieson, University of Washington (jamieson@cs.washington.edu)}
    \item \red{Gabor Lugosi,  Pompeu Fabra University, (gabor.lugosi@gmail.com)}
\end{itemize}

Reviewers:
\begin{itemize}
    \item \red{Yuxin Chen, University of Chicago (chenyuxin@uchicago.edu)}
    \item \red{Ray Li, UC Berkeley (rayyli@berkeley@edu)}
    \item \red{Daniel Golovin, Google, (Golovin@google.com)}
    \item \red{Rajan Udwani, UC Berkeley (rudwani@berkeley.edu)}
    \item \red{Lisa Hellerstein, New York University, (lisa.hellerstein@nyu.edu)}
\end{itemize}

Our submission has the following keywords: \red{submodular optimization}, \red{active learning}, \red{approximation algorithms}, \red{optimal decision tree}.

As the corresponding author, I confirm that none of the coauthors listed below have a conflict of interest with the action editors and referees I suggest above. Furthermore, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Su Jia (Cornell University)}\\
\red{Fatemeh Navidi (Aquatic Trading)}\\
\red{Viswanath Nagarajan (University of Michigan)}\\
\red{R. Ravi (Carnegie Mellon University)}

\end{document}
